Decision-Oriented Recommendation Reranking: An Empirical Study of Its Promise and Limitations

Large language models (LLMs) have shown promise for recommendation reranking, but their use introduces an important trade-off between recommendation quality and serving efficiency. We investigate whether decision-oriented systems provide a useful alternative when the reranking task is fundamentally a structured choice among predefined candidate items. Specifically, we conduct a controlled empirical study of two decision-oriented systems, TypeSafe Jev and OpenAI Decisions, for recommendation reranking. Across three Amazon Reviews domains and four candidate-set sizes, we compare these systems against recommendation-specific models and pointwise and listwise LLM-based rerankers, systematically evaluating recommendation effectiveness, candidate-order robustness, and efficiency and scalability. Our results reveal that Jev frequently achieves a favorable quality--latency trade-off, offering competitive recommendation effectiveness at substantially lower observed latency than stronger LLM-based alternatives. Overall, our findings suggest that specialization for decision-making does not inherently guarantee superior recommendation quality or robustness. Instead, the practical value of decision-oriented inference depends on implementation-specific characteristics and application requirements. These findings motivate further investigation of decision-oriented systems for recommendation and other ranking tasks with structured output spaces.

==> tab_fig/fig/b_pareto_number_input_100.tex <==
% K = 100
\addplot[
    color=black,
    line width=1pt,
    forget plot,
]
coordinates {
(0.001, 0.076)
(0.001, 0.082)
(0.170, 0.168)
(0.202, 0.191)
(3.320, 0.225)

};


\addplot[
    only marks,
    mark=text,
    text mark={\contour{black}{\textcolor{typesafe!80}{$\bigstar$}}},
%     mark=pentagon*,
%     mark options={solid,
%         fill=typesafe!80,
%         draw=black},
    mark size=4pt,
]
coordinates {

(0.202,0.191)

};         
         

\addplot[
    only marks,
    mark=pentagon*,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=4pt,
]
coordinates {

(0.170,0.168)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black,rotate=180},mark size=3pt,
]
coordinates {

(3.471,0.149)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=3pt,
]
coordinates {

(3.320,0.225)

};         
         

\addplot[
    only marks,
    mark=square*,
    mark options={solid,
        fill=yellow!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(7.495,0.115)

};         
         

\addplot[
    only marks,
    mark=stripedsquare,
    mark options={solid,
        fill=yellow!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.731,0.062)

};         
         

\addplot[
    only marks,
    mark=*,
    mark options={solid,
        fill=mutedred!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(31.086,0.072)

};         
         

\addplot[
    only marks,
    mark=stripedcircle,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(3.097,0.070)

};         
         

\addplot[
    only marks,
    mark=x,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.001,0.082)

};         
         

\addplot[
    only marks,
    mark=asterisk,
    mark options={solid,
        fill=mutedblue!80,
        draw=black},mark size=3pt,
]
coordinates {

        (0.001,0.076)

};         
        

==> tab_fig/fig/b_pareto_number_input_20.tex <==
% K = 20
\addplot[
    color=black,
    line width=1pt,
    forget plot,
]
coordinates {
(0.001, 0.187)
(0.137, 0.361)
(0.152, 0.406)
(1.274, 0.444)

};


\addplot[
    only marks,
    mark=text,
    text mark={\contour{black}{\textcolor{typesafe!80}{$\bigstar$}}},
%     mark=pentagon*,
%     mark options={solid,
%         fill=typesafe!80,
%         draw=black},
    mark size=4pt,
]
coordinates {

(0.152,0.406)

};         
         

\addplot[
    only marks,
    mark=pentagon*,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=4pt,
]
coordinates {

(0.137,0.361)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black,rotate=180},mark size=3pt,
]
coordinates {

(1.399,0.397)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=3pt,
]
coordinates {

(1.274,0.444)

};         
         

\addplot[
    only marks,
    mark=square*,
    mark options={solid,
        fill=yellow!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(1.525,0.347)

};         
         

\addplot[
    only marks,
    mark=stripedsquare,
    mark options={solid,
        fill=yellow!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.193,0.293)

};         
         

\addplot[
    only marks,
    mark=*,
    mark options={solid,
        fill=mutedred!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(6.222,0.295)

};         
         

\addplot[
    only marks,
    mark=stripedcircle,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.799,0.351)

};         
         

\addplot[
    only marks,
    mark=x,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.001,0.082)

};         
         

\addplot[
    only marks,
    mark=asterisk,
    mark options={solid,
        fill=mutedblue!80,
        draw=black},mark size=3pt,
]
coordinates {

        (0.001,0.187)

};      

==> tab_fig/fig/b_pareto_number_input_200.tex <==
% K = 200
\addplot[
    color=black,
    line width=1pt,
    forget plot,
]
coordinates {
(0.001, 0.062)
(0.001, 0.082)
(0.193, 0.121)
(0.264, 0.152)
(6.384, 0.183)

};


\addplot[
    only marks,
    mark=text,
    text mark={\contour{black}{\textcolor{typesafe!80}{$\bigstar$}}},
%     mark=pentagon*,
%     mark options={solid,
%         fill=typesafe!80,
%         draw=black},
    mark size=4pt,
]
coordinates {

(0.264,0.152)

};         
         

\addplot[
    only marks,
    mark=pentagon*,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=4pt,
]
coordinates {

(0.193,0.121)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black,rotate=180},mark size=3pt,
]
coordinates {

(12.449,0.071)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=3pt,
]
coordinates {

(6.384,0.183)

};         
         

\addplot[
    only marks,
    mark=square*,
    mark options={solid,
        fill=yellow!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(14.868,0.080)

};         
         

\addplot[
    only marks,
    mark=stripedsquare,
    mark options={solid,
        fill=yellow!80,
        draw=black},mark size=3pt,
]
coordinates {

(1.530,0.030)

};         
         

\addplot[
    only marks,
    mark=*,
    mark options={solid,
        fill=mutedred!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(62.315,0.041)

};         
         

\addplot[
    only marks,
    mark=stripedcircle,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(6.330,0.034)

};         
         

\addplot[
    only marks,
    mark=x,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.001,0.082)

};         
         

\addplot[
    only marks,
    mark=asterisk,
    mark options={solid,
        fill=mutedblue!80,
        draw=black},mark size=3pt,
]
coordinates {

        (0.001,0.062)

};         

==> tab_fig/fig/b_pareto_number_input_50.tex <==
% K = 50
\addplot[
    color=black,
    line width=1pt,
    forget plot,
]
coordinates {
(0.001, 0.102)
(0.148, 0.227)
(0.163, 0.263)
(2.021, 0.310)

};


\addplot[
    only marks,
    mark=text,
    text mark={\contour{black}{\textcolor{typesafe!80}{$\bigstar$}}},
%     mark=pentagon*,
%     mark options={solid,
%         fill=typesafe!80,
%         draw=black},
    mark size=4pt,
]
coordinates {

(0.163,0.263)

};         
         

\addplot[
    only marks,
    mark=pentagon*,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=4pt,
]
coordinates {

(0.148,0.227)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black,rotate=180},mark size=3pt,
]
coordinates {

(2.107,0.246)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=3pt,
]
coordinates {

(2.021,0.310)

};         
         

\addplot[
    only marks,
    mark=square*,
    mark options={solid,
        fill=yellow!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(3.769,0.189)

};         
         

\addplot[
    only marks,
    mark=stripedsquare,
    mark options={solid,
        fill=yellow!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.390,0.138)

};         
         

\addplot[
    only marks,
    mark=*,
    mark options={solid,
        fill=mutedred!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(15.565,0.136)

};         
         

\addplot[
    only marks,
    mark=stripedcircle,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(1.629,0.163)

};         
         

\addplot[
    only marks,
    mark=x,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.001,0.082)

};         
         

\addplot[
    only marks,
    mark=asterisk,
    mark options={solid,
        fill=mutedblue!80,
        draw=black},mark size=3pt,
]
coordinates {

        (0.001,0.102)

};   

==> tab_fig/fig/mt_pareto_number_input_100.tex <==
% K = 100
\addplot[
    color=black,
    line width=1pt,
    forget plot,
]
coordinates {
(0.001, 0.084)
(0.001, 0.095)
(0.179, 0.117)
(4.645, 0.140)

};


\addplot[
    only marks,
    mark=text,
    text mark={\contour{black}{\textcolor{typesafe!80}{$\bigstar$}}},
%     mark=pentagon*,
%     mark options={solid,
%         fill=typesafe!80,
%         draw=black},
    mark size=4pt,
]
coordinates {

(0.179,0.117)

};         
         

\addplot[
    only marks,
    mark=pentagon*,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=4pt,
]
coordinates {

(0.146,0.087)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black,rotate=180},mark size=3pt,
]
coordinates {

(2.370,0.087)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=3pt,
]
coordinates {

(4.645,0.140)

};         
         

\addplot[
    only marks,
    mark=square*,
    mark options={solid,
        fill=yellow!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(3.045,0.093)

};         
         

\addplot[
    only marks,
    mark=stripedsquare,
    mark options={solid,
        fill=yellow!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.202,0.058)

};         
         

\addplot[
    only marks,
    mark=*,
    mark options={solid,
        fill=mutedred!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(12.466,0.055)

};         
         

\addplot[
    only marks,
    mark=stripedcircle,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.887,0.062)

};         
         

\addplot[
    only marks,
    mark=x,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.001,0.095)

};         
         

\addplot[
    only marks,
    mark=asterisk,
    mark options={solid,
        fill=mutedblue!80,
        draw=black},mark size=3pt,
]
coordinates {

        (0.001,0.084)

};         

==> tab_fig/fig/mt_pareto_number_input_20.tex <==
% K = 20
\addplot[
    color=black,
    line width=1pt,
    forget plot,
]
coordinates {
(0.001, 0.172)
(0.064, 0.247)
(0.092, 0.262)
(0.155, 0.293)
(1.450, 0.307)

};


\addplot[
    only marks,
    mark=text,
    text mark={\contour{black}{\textcolor{typesafe!80}{$\bigstar$}}},
%     mark=pentagon*,
%     mark options={solid,
%         fill=typesafe!80,
%         draw=black},
    mark size=4pt,
]
coordinates {

(0.155,0.293)

};         
         
\addlegendentry{Jev}
        

\addplot[
    only marks,
    mark=pentagon*,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=4pt,
]
coordinates {

(0.092,0.262)

};         
         
\addlegendentry{Decisions}        
        

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black,rotate=180},mark size=3pt,
]
coordinates {

(1.320,0.288)

};         
         
\addlegendentry{GPT-6-Luna (L)}        
        

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=3pt,
]
coordinates {

(1.450,0.307)

};         
         
\addlegendentry{GPT-6-Sol (L)}        
        

\addplot[
    only marks,
    mark=square*,
    mark options={solid,
        fill=yellow!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(0.607,0.289)

};         
         
\addlegendentry{Qwen2.5 7B (P)}
        

\addplot[
    only marks,
    mark=stripedsquare,
    mark options={solid,
        fill=yellow!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.064,0.247)

};         
         
\addlegendentry{Qwen2.5 7B (L)}        
        

\addplot[
    only marks,
    mark=*,
    mark options={solid,
        fill=mutedred!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(2.521,0.267)

};         
         
\addlegendentry{Qwen2.5 32B (P)}
        

\addplot[
    only marks,
    mark=stripedcircle,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.280,0.254)

};         
         
\addlegendentry{Qwen2.5 32B (L)}        
        

\addplot[
    only marks,
    mark=x,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.001,0.096)

};         
         
\addlegendentry{SASRec}        
        

\addplot[
    only marks,
    mark=asterisk,
    mark options={solid,
        fill=mutedblue!80,
        draw=black},mark size=3pt,
]
coordinates {

        (0.001,0.172)

};         
         
\addlegendentry{DCNv2}  

==> tab_fig/fig/mt_pareto_number_input_200.tex <==
% K = 200
\addplot[
    color=black,
    line width=1pt,
    forget plot,
]
coordinates {
(0.001, 0.075)
(0.001, 0.096)
(6.778, 0.099)

};


\addplot[
    only marks,
    mark=text,
    text mark={\contour{black}{\textcolor{typesafe!80}{$\bigstar$}}},
%     mark=pentagon*,
%     mark options={solid,
%         fill=typesafe!80,
%         draw=black},
    mark size=4pt,
]
coordinates {

(0.198,0.077)

};         
         

\addplot[
    only marks,
    mark=pentagon*,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=4pt,
]
coordinates {

(0.161,0.053)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black,rotate=180},mark size=3pt,
]
coordinates {

(3.995,0.043)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=3pt,
]
coordinates {

(6.778,0.099)

};         
         

\addplot[
    only marks,
    mark=square*,
    mark options={solid,
        fill=yellow!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(6.073,0.059)

};         
         

\addplot[
    only marks,
    mark=stripedsquare,
    mark options={solid,
        fill=yellow!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.398,0.034)

};         
         

\addplot[
    only marks,
    mark=*,
    mark options={solid,
        fill=mutedred!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(24.925,0.037)

};         
         

\addplot[
    only marks,
    mark=stripedcircle,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(1.657,0.033)

};         
         

\addplot[
    only marks,
    mark=x,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.001,0.096)

};         
         

\addplot[
    only marks,
    mark=asterisk,
    mark options={solid,
        fill=mutedblue!80,
        draw=black},mark size=3pt,
]
coordinates {

        (0.001,0.075)

};         

==> tab_fig/fig/mt_pareto_number_input_50.tex <==
% K = 50
\addplot[
    color=black,
    line width=1pt,
    forget plot,
]
coordinates {
(0.001, 0.107)
(0.120, 0.118)
(0.136, 0.132)
(0.159, 0.162)
(2.722, 0.178)

};


\addplot[
    only marks,
    mark=text,
    text mark={\contour{black}{\textcolor{typesafe!80}{$\bigstar$}}},
%     mark=pentagon*,
%     mark options={solid,
%         fill=typesafe!80,
%         draw=black},
    mark size=4pt,
]
coordinates {

(0.159,0.162)

};         
         

\addplot[
    only marks,
    mark=pentagon*,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=4pt,
]
coordinates {

(0.136,0.132)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black,rotate=180},mark size=3pt,
]
coordinates {

(1.762,0.143)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=3pt,
]
coordinates {

(2.722,0.178)

};         
         

\addplot[
    only marks,
    mark=square*,
    mark options={solid,
        fill=yellow!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(1.526,0.151)

};         
         

\addplot[
    only marks,
    mark=stripedsquare,
    mark options={solid,
        fill=yellow!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.120,0.118)

};         
         

\addplot[
    only marks,
    mark=*,
    mark options={solid,
        fill=mutedred!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(6.252,0.117)

};         
         

\addplot[
    only marks,
    mark=stripedcircle,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.501,0.124)

};         
         

\addplot[
    only marks,
    mark=x,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.001,0.096)

};         
         

\addplot[
    only marks,
    mark=asterisk,
    mark options={solid,
        fill=mutedblue!80,
        draw=black},mark size=3pt,
]
coordinates {

        (0.001,0.107)

};       

==> tab_fig/fig/vg_pareto_number_input_100.tex <==
% K = 100
\addplot[
    color=black,
    line width=1pt,
    forget plot,
]
coordinates {
(0.001, 0.065)
(0.001, 0.081)
(0.172, 0.128)
(0.210, 0.153)
(4.472, 0.175)

};


\addplot[
    only marks,
    mark=text,
    text mark={\contour{black}{\textcolor{typesafe!80}{$\bigstar$}}},
%     mark=pentagon*,
%     mark options={solid,
%         fill=typesafe!80,
%         draw=black},
    mark size=4pt,
]
coordinates {

(0.210,0.153)

};         
         

\addplot[
    only marks,
    mark=pentagon*,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=4pt,
]
coordinates {

(0.172,0.128)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black,rotate=180},mark size=3pt,
]
coordinates {

(3.209,0.123)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=3pt,
]
coordinates {

(4.472,0.175)

};         
         

\addplot[
    only marks,
    mark=square*,
    mark options={solid,
        fill=yellow!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(7.267,0.119)

};         
         

\addplot[
    only marks,
    mark=stripedsquare,
    mark options={solid,
        fill=yellow!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.688,0.059)

};         
         

\addplot[
    only marks,
    mark=*,
    mark options={solid,
        fill=mutedred!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(29.905,0.064)

};         
         

\addplot[
    only marks,
    mark=stripedcircle,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(2.892,0.062)

};         
         

\addplot[
    only marks,
    mark=x,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.001,0.081)

};         
         

\addplot[
    only marks,
    mark=asterisk,
    mark options={solid,
        fill=mutedblue!80,
        draw=black},mark size=3pt,
]
coordinates {

        (0.001,0.065)

};    

==> tab_fig/fig/vg_pareto_number_input_20.tex <==
% K = 20
\addplot[
    color=black,
    line width=1pt,
    forget plot,
]
coordinates {
(0.001, 0.157)
(0.135, 0.331)
(0.155, 0.360)
(1.552, 0.380)

};


\addplot[
    only marks,
    mark=text,
    text mark={\contour{black}{\textcolor{typesafe!80}{$\bigstar$}}},
%     mark=pentagon*,
%     mark options={solid,
%         fill=typesafe!80,
%         draw=black},
    mark size=4pt,
]
coordinates {

(0.155,0.360)

};         
         

\addplot[
    only marks,
    mark=pentagon*,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=4pt,
]
coordinates {

(0.135,0.331)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black,rotate=180},mark size=3pt,
]
coordinates {

(1.500,0.327)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=3pt,
]
coordinates {

(1.552,0.380)

};         
         

\addplot[
    only marks,
    mark=square*,
    mark options={solid,
        fill=yellow!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(1.480,0.321)

};         
         

\addplot[
    only marks,
    mark=stripedsquare,
    mark options={solid,
        fill=yellow!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.181,0.263)

};         
         

\addplot[
    only marks,
    mark=*,
    mark options={solid,
        fill=mutedred!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(6.063,0.283)

};         
         

\addplot[
    only marks,
    mark=stripedcircle,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.767,0.297)

};         
         

\addplot[
    only marks,
    mark=x,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.001,0.081)

};         
         

\addplot[
    only marks,
    mark=asterisk,
    mark options={solid,
        fill=mutedblue!80,
        draw=black},mark size=3pt,
]
coordinates {

        (0.001,0.157)

};        

==> tab_fig/fig/vg_pareto_number_input_200.tex <==
% K = 200
\addplot[
    color=black,
    line width=1pt,
    forget plot,
]
coordinates {
(0.001, 0.054)
(0.001, 0.081)
(0.196, 0.093)
(0.293, 0.107)
(9.023, 0.122)

};


\addplot[
    only marks,
    mark=text,
    text mark={\contour{black}{\textcolor{typesafe!80}{$\bigstar$}}},
%     mark=pentagon*,
%     mark options={solid,
%         fill=typesafe!80,
%         draw=black},
    mark size=4pt,
]
coordinates {

(0.293,0.107)

};         
         

\addplot[
    only marks,
    mark=pentagon*,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=4pt,
]
coordinates {

(0.196,0.093)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black,rotate=180},mark size=3pt,
]
coordinates {

(11.973,0.047)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=3pt,
]
coordinates {

(9.023,0.122)

};         
         

\addplot[
    only marks,
    mark=square*,
    mark options={solid,
        fill=yellow!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(14.555,0.078)

};         
         

\addplot[
    only marks,
    mark=stripedsquare,
    mark options={solid,
        fill=yellow!80,
        draw=black},mark size=3pt,
]
coordinates {

(1.448,0.025)

};         
         

\addplot[
    only marks,
    mark=*,
    mark options={solid,
        fill=mutedred!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(60.383,0.040)

};         
         

\addplot[
    only marks,
    mark=stripedcircle,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(5.798,0.039)

};         
         

\addplot[
    only marks,
    mark=x,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.001,0.081)

};         
         

\addplot[
    only marks,
    mark=asterisk,
    mark options={solid,
        fill=mutedblue!80,
        draw=black},mark size=3pt,
]
coordinates {

        (0.001,0.054)

};         
         

==> tab_fig/fig/vg_pareto_number_input_50.tex <==
% K = 50
\addplot[
    color=black,
    line width=1pt,
    forget plot,
]
coordinates {
(0.001, 0.090)
(0.147, 0.197)
(0.175, 0.228)
(2.628, 0.241)

};


\addplot[
    only marks,
    mark=text,
    text mark={\contour{black}{\textcolor{typesafe!80}{$\bigstar$}}},
%     mark=pentagon*,
%     mark options={solid,
%         fill=typesafe!80,
%         draw=black},
    mark size=4pt,
]
coordinates {

(0.175,0.228)

};         
         

\addplot[
    only marks,
    mark=pentagon*,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=4pt,
]
coordinates {

(0.147,0.197)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black,rotate=180},mark size=3pt,
]
coordinates {

(2.389,0.178)

};         
         

\addplot[
    only marks,
    mark=stripedtriangle,
    mark options={solid,
        fill=mutedblue,
        draw=black},mark size=3pt,
]
coordinates {

(2.628,0.241)

};         
         

\addplot[
    only marks,
    mark=square*,
    mark options={solid,
        fill=yellow!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(3.645,0.175)

};         
         

\addplot[
    only marks,
    mark=stripedsquare,
    mark options={solid,
        fill=yellow!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.368,0.106)

};         
         

\addplot[
    only marks,
    mark=*,
    mark options={solid,
        fill=mutedred!80,
        draw=black},
        mark size=3pt,
]
coordinates {

(15.167,0.117)

};         
         

\addplot[
    only marks,
    mark=stripedcircle,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(1.551,0.122)

};         
         

\addplot[
    only marks,
    mark=x,
    mark options={solid,
        fill=mutedred!80,
        draw=black},mark size=3pt,
]
coordinates {

(0.001,0.081)

};         
         

\addplot[
    only marks,
    mark=asterisk,
    mark options={solid,
        fill=mutedblue!80,
        draw=black},mark size=3pt,
]
coordinates {

        (0.001,0.090)

};    
